Early Risk Detection of Pathological Gambling, Self-Harm and Depression Using BERT

Early risk detection of mental illnesses has a massive positive impact upon the well-being of people. The eRisk workshop has been at the forefront of enabling interdisciplinary research in developing computational methods to automatically estimate early risk factors for mental issues such as depression, self-harm, anorexia and pathological gambling. In this paper, we present the contributions of the BLUE team in the 2021 edition of the workshop, in which we tackle the problems of early detection of gambling addiction, self-harm and estimating depression severity from social media posts. We employ pre-trained BERT transformers and data crawled automatically from mental health subreddits and obtain reasonable results on all three tasks.

==> sections/tables.tex <==
\begin{table}[hbt!]
    \centering
    \resizebox{0.75\textwidth}{!}{
        \begin{tabular}{lccccccccc}
        \hline team name & run id & P & R & F1 & ERDE$_5$ & ERDE$_{50}$ & latency$_{TP}$ & speed & latency-weighted F1 \\
        \hline
        UNSL & 0 & .326 & .957 & .487 & .079 & .023 & 11 & .961 & .468 \\
        UNSL & 1 & .137 & .982 & .241 & .060 & .035 & 4 & .988 & .238 \\
        UNSL & 2 & .586 & .939 & .721 & .073 & .020 & 11 & .961 & .693 \\
        UNSL & 3 & .084 & .963 & .155 & .066 & .060 & 1 &  1 & .155 \\
        UNSL & 4 & .086 & .933 & .157 & .067 & .060 & 1 &  1 & .157 \\
        RELAI & 0 & .138 & .988 & .243 & .048 & .036 & 1 &  1 & .243 \\
        RELAI & 1 & .108 & 1 & .194 & .057 & .045 & 1 &  1 & .194 \\
        RELAI & 2 & .071 & 1 & .132 & .067 & .064 & 1 &  1 & .132 \\
        RELAI & 3 & .071 & 1 & .132 & .066 & .064 & 1 &  1 & .132 \\
        RELAI & 4 & .070 & 1 & .131 & .066 & .065 & 1 &  1 & .131 \\
        BLUE & 0 & .107 & .994 & .193 & .067 & .046 & 2 &  .996 & .192 \\
        BLUE & 1 & .157 & .988 & .271 & .054 & .036 & 2 &  .996 & .270 \\
        BLUE & 2 & .121 & .994 & .215 & .065 & .045 & 2 &  .996 & .215 \\
        BLUE & 3 & .095 & 1 & .174 & .071 & .051 & 2 &  .996 & .173 \\
        BLUE & 4 & .110 & .994 & .198 & .068 & .048 & 2 &  .996 & .197 \\
        UPV-Symanto & 0 & .042 & .415 & .077 & .088 & .087 & 1 & 1 & .077 \\
        UPV-Symanto & 1 & .040 & .457 & .074 & .097 & .091 & 1 & 1 & .074 \\
        UPV-Symanto & 2 & .030 & .238 & .053 & .093 & .091 & 1 & 1 & .053 \\
        UPV-Symanto & 3 & .035 & .409 & .064 & .098 & .097 & 1 & 1 & .064 \\
        UPV-Symanto & 4 & .028 & .256 & .051 & .098 & .095 & 1 & 1 & .051 \\
        CeDRI & 0 & .076 & 1 & .142 & .079 & .060 & 2 &  .996 & .141 \\
        CeDRI & 1 & .070 & 1 & .131 & .066 & .065 & 1 &  1 & .131 \\
        EFE & 0 & .251 & .640 & .361 & .079 & .037 & 16 & .942 & .340 \\
        EFE & 1 & .296 & .537 & .382 & .076 & .043 & 31 & .884 & .337 \\
        EFE & 2 & .233 & .750 & .356 & .082 & .033 & 11 & .961 & .342 \\
        EFE & 3 & .292 & .549 & .381 & .076 & .044 & 31 & .884 & .337 
        \end{tabular}
    }
    \caption{Decision-based evaluation on Task 1: Early Detection of Signs of Pathological Gambling. }
    \label{tab:task1-results}
\end{table}

\begin{table}[hbt!]
    \centering
    \resizebox{0.75\textwidth}{!}{
        \begin{tabular}{lccccccccc}
        \hline team name & run id & P & R & F1 & ERDE$_5$ & ERDE$_{50}$ & latency$_{TP}$ & speed & latency-weighted F1 \\
        \hline
            NLP-UNED & 0 & .442 & .75 & .556 & .08 & .042 & 6 & .981 & .545 \\
            NLP-UNED & 1 & .442 & .796 & .568 & .091 & .041 & 11 & .961 & .546 \\
            NLP-UNED & 2 & .422 & .73 & .535 & .088 & .047 & 7 & .977 & .522 \\
            NLP-UNED & 3 & .419 & .77 & .543 & .093 & .047 & 10 & .965 & .524 \\
            NLP-UNED & 4 & .453 & .816 & .582 & .088 & .04 & 9 & .969 & .564 \\
            AvocadoToast & 0 & .214 & .757 & .334 & .111 & .069 & 11 & .961 & .321 \\
            AvocadoToast & 1 & .245 & .401 & .304 & .078 & .076 & 11 &.0 & .304 \\
            AvocadoToast & 2 & .215 & .757 & .335 & .111 & .069 & 11 & .961 & .322 \\
            Birmingham & 0 & .584 & .526 & .554 & .068 & .054 & 2 & .996 & .551  \\
            Birmingham & 1 & .644 & .309 & .418 & .097 & .074 & 8 & .973 & .406  \\
            Birmingham & 2 & .757 & .349 & .477 & .085 & .07 & 4 & .988 & .472  \\
            Birmingham & 3 & .629 & .434 & .514 & .084 & .062 & 5 & .984 & .506  \\
            Birmingham & 4 & .0 & .0 & .0 & .105 & .105  \\
            NuFAST & 0 & .124 & .283 & .172 & .101 & .097 & 1 & 1.0 & .172 \\
            NuFAST & 1 & .124 & .283 & .172 & .101 & .097 & 1 & 1.0 & .172 \\
            NuFAST & 2 & .124 & .283 & .172 & .101 & .097 & 1 & 1.0 & .172 \\
            NaCTeM & 0 & .108 & .882 & .193 & .185 & .184 & 1999 & .0 & .0 \\
            NaCTeM & 1 & .108 & .882 & .193 & .185 & .184 & 1999 & .0 & .0 \\
            NaCTeM & 2 & .108 & .882 & .193 & .185 & .184 & 1999 & .0 & .0 \\
            NaCTeM & 3 & .108 & .882 & .193 & .184 & .184 & 1999 & .0 & .0 \\
            NaCTeM & 4 & .108 & .882 & .193 & .184 & .184 & 1999 & .0 & .0 \\
            EFE & 0 & .381 & .717 & .498 & .118 & .05 & 17 & .938 & .467 \\
            EFE & 1 & .434 & .605 & .505 & .114 & .063 & 32 & .88 & .445 \\
            EFE & 2 & .366 & .796 & .501 & .12 & .043 & 12 & .957 & .48 \\
            EFE & 3 & .422 & .605 & .497 & .114 & .063 & 32 & .88 & .437 \\
            BioInfo@UAVR & 0 & .233 & .862 & .367 & .136 & .05 & 22 & .918 & .337 \\
            BioInfo@UAVR & 1 & .274 & .789 & .407 & .128 & .047 & 22 & .918 & .374 \\
            NUS-IDS & 0 & .133 & .987 & .234 & .108 & .073 & 3 & .992 & .232 \\
            NUS-IDS & 1 & .131 & .98 & .232 & .116 & .073 & 4 & .988 & .229 \\
            NUS-IDS & 2 & .134 & .993 & .236 & .117 & .072 & 4 & .988 & .233 \\
            NUS-IDS & 3 & .128 & .987 & .227 & .106 & .075 & 3 & .992 & .225 \\
            NUS-IDS & 4 & .135 & .987 & .237 & .104 & .071 & 3 & .992 & .235 \\
            RELAI & 0 & .138 & .967 & .242 & .14 & .073 & 5 & .984 & .238  \\
            RELAI & 1 & .114 & .993 & .205 & .146 & .086 & 5 & .984 & .202  \\
            RELAI & 2 & .488 & .276 & .353 & .087 & .082 & 2 & .996 & .352  \\
            RELAI & 3 & .207 & .875 & .335 & .079 & .056 & 2 & .996 & .334  \\
            RELAI & 4 & .119 & .868 & .209 & .12 & .089 & 2 & .996 & .208  \\
            CeDRI & 0 & .11 & .993 & .199 & .109 & .09 & 2 & .996 & .198  \\
            CeDRI & 1 & .116 & 1.0 & .207 & .113 & .085 & 2 & .996 & .206 \\
            CeDRI & 2 & .105 & 1.0 & .19 & .096 & .094 & 1 & 1.0 & .19 \\
            BLUE & 0 & .283 & .934 & .435 & .084 & .041 & 5 & .984 & .428  \\
            BLUE & 1 & .142 & .875 & .245 & .117 & .081 & 4 & .988 & .242  \\
            BLUE & 2 & .454 & .849 & .592 & .079 & .037 & 7 & .977 & .578  \\
            BLUE & 3 & .394 & .868 & .542 & .075 & .035 & 5 & .984 & .534  \\
            BLUE & 4 & .249 & .928 & .393 & .085 & .044 & 4 & .988 & .388  \\
            UPV-Symanto & 0 & .307 & .678 & .422 & .097 & .051 & 5 & .984 & .416 \\
            UPV-Symanto & 1 & .276 & .638 & .385 & .059 & .056 & 1 & 1 &.0 .385 \\
            UPV-Symanto & 2 & .313 & .645 & .422 & .072 & .053 & 2 & .996 & .42 \\
            UPV-Symanto & 3 & .301 & .77 & .433 & .089 & .044 & 5 & .984 & .426 \\
            UPV-Symanto & 4 & .198 & .711 & .31 & .082 & .063 & 3 & .992 & .307 \\
            UNSL & 0 & .336 & .914 & .491 & .125 & .034 & 11 & .961 & .472  \\
            UNSL & 1 & .11 & .987 & .198 & .093 & .092 & 1 & 1.0 & .198 \\
            UNSL & 2 & .129 & .934 & .226 & .098 & .085 & 1 & 1.0 & .226 \\
            UNSL & 3 & .464 & .803 & .588 & .064 & .038 & 3 & .992 & .583  \\
            UNSL & 4 & .532 & .763 & .627 & .064 & .038 & 3 & .992 & .622 
        \end{tabular}
    }
    \caption{Decision-based results for Task 2: Early Detection of Signs of Self-Harm. }
    \label{tab:task2-results}
\end{table}

\begin{table}[hbt!]
    \centering
    \resizebox{0.75\textwidth}{!}{
        \begin{tabular}{lcccc}
        \hline Run & AHR & ACR & ADODL & DCHR \\
        \hline BLUE run0 & $27.86 \%$ & $64.66 \%$ & $74.15 \%$ & $17.50 \%$ \\
            BLUE run1 & $30.00 \%$ & $64.58 \%$ & $70.65 \%$ & $11.25 \%$ \\
            BLUE run2 & $30.36 \%$ & $65.42 \%$ & $75.42 \%$ & $21.25 \%$ \\
            BLUE run3 & $29.52 \%$ & $64.70 \%$ & $73.63 \%$ & $13.75 \%$ \\
            BLUE run4 & $29.76 \%$ & $65.04 \%$ & $74.84 \%$ & $15.00 \%$  \\
            CYUT run1 & 32.02\% & 66.33\% & 75.34\% & 20.00\% \\
            CYUT run2 & 32.62\% & 69.46\% & 83.59\% & 41.25\% \\
            CYUT run3 & 28.39\% & 63.51\% & 80.10\% & 38.75\% \\
            DUTH\_ATHENA MaxFT & 31.43\% & 64.86\% & 74.46\% & 15.00\% \\
            DUTH\_ATHENA MeanFT & 32.02\% & 65.63\% & 73.81\% & 12.50\% \\
            DUTH\_ATHENA MeanPosts & 25.06\% & 63.97\% & 80.28\% & 30.00\% \\
            DUTH\_ATHENA MeanPostsAB & 33.04\% & 67.86\% & 80.32\% & 27.50\% \\
            DUTH\_ATHENA MeanPostsSVM & 35.36\% & 67.18\% & 73.97\% & 15.00\% \\
            NaCTeM run1 & 31.43\% & 64.54\% & 74.98\% & 18.75\% \\
            NaCTeM run2 & 31.55\% & 65.00\% & 75.04\% & 21.25\% \\
            NaCTeM run3 & 32.86\% & 66.67\% & 76.23\% & 22.50\% \\
            RELAI dmknn\_dan & 34.64\% & 67.58\% & 78.69\% & 23.75\% \\
            RELAI dmknn\_danb & 30.18\% & 65.26\% & 78.91\% & 25.00\% \\
            RELAI etm & 38.78\% & 72.56\% & 80.27 \% & 35.71\%∗ \\
            RELAI k\_nn dan & 34.82\% & 66.07\% & 72.38\% & 11.25\% \\
            RELAI lda & 28.33\% & 63.19\% & 68.00\% & 10.00\% \\
            Tanvi Darci run 1 & 35.12\% & 67.76\% & 75.81\% & 22.50\% \\
            Unior\_NLP uniorA & 31.67\% & 63.95\% & 69.42\% & 08.75\% \\
            Unior\_NLP uniorB & 31.61\% & 64.66\% & 74.74\% & 15.00\% \\
            Unior\_NLP uniorC & 28.63\% & 63.31\% & 76.45\% & 20.00\% \\
            Unior\_NLP uniorD & 28.10\% & 64.25\% & 71.27\% & 15.00\% \\
            uOttawa1\_sim\_BERT\_base+ & 28.39\% & 65.73\% & 78.91\% & 25.00\% \\
            uOttawa2\_Top2Vec\_USE+ & 28.04\% & 63.00\% & 77.32\% & 27.50\% \\
            uOttawa3\_sim\_BERT\_large+ & 25.83\% & 59.68\% & 71.23\% & 27.50\% \\
            uOttawa4\_Ensemble\_BERT\_QA & 27.68\% & 62.08\% & 76.92\% & 20.00\% \\
            uOttawa5\_sim\_ROBERTA+ & 26.31\% & 62.60\% & 76.45\% & 30.00\% \\
            UPV-Symanto 0\_symanto\_upv\_svm\_linear\_drb & 34.58\% & 67.32\% & 75.62\% & 26.25\% \\
            UPV-Symanto 1\_symanto\_upv\_svm\_linear\_mt30 & 32.20\% & 66.05\% & 77.28\% & 26.25\% \\
            UPV-Symanto 2\_symanto\_upv\_svm\_linear & 33.15\% & 66.05\% & 75.42\% & 23.75\% \\
            UPV-Symanto 3\_symanto\_upv\_rfc\_df40\_mt30 & 33.09\% & 66.39\% & 76.87\% & 23.75\% \\
            UPV-Symanto 4\_symanto\_upv\_lingfeat\_cors & 34.17\% & 73.17\% & 82.42\% & 32.50\% \\
        \end{tabular}
    }
    \caption{Competition results for \textbf{Task 3}: Measuring the severity of the signs of depression. Best results are obtained through similarity learning.}
    \label{tab:task3-results}
\end{table}



